CLIP-Fields: Weakly Supervised Semantic Fields for Robotic Memory

We propose CLIP-Fields, an implicit scene model that can be used for a variety of tasks, such as segmentation, instance identification, semantic search over space, and view localization. CLIP-Fields learns a mapping from spatial locations to semantic embedding vectors. Importantly, we show that this mapping can be trained with supervision coming only from web-image and web-text trained models such as CLIP, Detic, and Sentence-BERT; and thus uses no direct human supervision. When compared to baselines like Mask-RCNN, our method outperforms on few-shot instance identification or semantic segmentation on the HM3D dataset with only a fraction of the examples. Finally, we show that using CLIP-Fields as a scene memory, robots can perform semantic navigation in real-world environments. Our code and demonstration videos are available here: https://mahis.life/clip-fields

==> 05robot.tex <==

\begin{figure*}
\includegraphics[width=\textwidth]{figures/robot_examples_v01.pdf}
\vskip 0.15cm
\includegraphics[width=\textwidth]{figures/robot_views_v01.pdf}
\caption{Examples of the Hello Robot Stretch in two different testing environments, looking at objects given different commands. The top row shows an exterior view of the robot in its environment, while the bottom shows an example from the robot's perspective. From left to right: ``sink'', ``microwave'', ``typewriter'', and ``plant.'' Scenes were either in a lab kitchen or in our lab's library/lounge space.
}
\end{figure*}

==> acknowledgements.tex <==
\section{Acknowledgements}
We thank AWS for computing resources and Boren Tsai for support in setting up the robot. We also gratefully acknowledge the support from Komatsu Ltd., The Open Philanthropy Project, Berkeley DeepDrive, NSF, and the ONR Pecase award.
